Unleashing the Power of Multi-Task Learning: A Comprehensive Survey Spanning Traditional, Deep, and Pretrained Foundation Model Eras

MTL is a learning paradigm that effectively leverages both task-specific and shared information to address multiple related tasks simultaneously. In contrast to STL, MTL offers a suite of benefits that enhance both the training process and the inference efficiency. MTL's key advantages encompass streamlined model architecture, performance enhancement, and cross-domain generalizability. Over the past twenty years, MTL has become widely recognized as a flexible and effective approach in various fields, including CV, NLP, recommendation systems, disease prognosis and diagnosis, and robotics. This survey provides a comprehensive overview of the evolution of MTL, encompassing the technical aspects of cutting-edge methods from traditional approaches to deep learning and the latest trend of pretrained foundation models. Our survey methodically categorizes MTL techniques into five key areas: regularization, relationship learning, feature propagation, optimization, and pre-training. This categorization not only chronologically outlines the development of MTL but also dives into various specialized strategies within each category. Furthermore, the survey reveals how the MTL evolves from handling a fixed set of tasks to embracing a more flexible approach free from task or modality constraints. It explores the concepts of task-promptable and -agnostic training, along with the capacity for ZSL, which unleashes the untapped potential of this historically coveted learning paradigm. Overall, we hope this survey provides the research community with a comprehensive overview of the advancements in MTL from its inception in 1997 to the present in 2023. We address present challenges and look ahead to future possibilities, shedding light on the opportunities and potential avenues for MTL research in a broad manner. This project is publicly available at https://github.com/junfish/Awesome-Multitask-Learning.

==> table_files/deep_summary_fix.tex <==
\begin{table*}[t]
    \centering
    \tiny
    % \scriptsize
    % \small
    \caption{Summary of deep MTL models.} %\jun{Inspired by "model card"\citeyear{mitchell2019model}
    \midsepremove
    \scalebox{0.5}{
    \begin{threeparttable}
    \begin{tabular}{p{0.7in}p{0.5in}p{0.3in}p{1.0in}p{0.3in}p{0.3in}p{0.3in}p{2.0in}p{1.5in}p{1.0in}p{0.6in}}
    
    \rowcolor{gray!40}
    \toprule
        Model Name & Origin & Year & MTL Strategy & Backbone & Sharing & Modality & Task & Measurement & Loss Function & Availability\tnote{1}\\
    \toprule % TCDCN
         TCDCN & ECCV & \citeyear{zhang2014facial} & Early stopping & CNN & Hard & Image & Facial landmark detection/head pose estimation/gender classification/age estimation/expression recognition/facial attribute inference & Mean error (mErr)~\citep{burgos2013robust}, failure rate~\citeyear{dantone2012real} & Mean squared error (MSE), cross-entropy (CE) loss & \href{http://mmlab.ie.cuhk.edu.hk/projects/TCDCN.html}{\textcolor{citegreen}{Official}} \\
         
    \midrule % MTL-MLT
    \rowcolor{gray!20}
         MTL-ML & ACL-IJCNLP & \citeyear{dong2015multi} & --- & RNN & Hard & Text & Multiple-target language translation & BLEU-4~\citep{papineni2002bleu}, Delta & CE loss & ---\\
    
    
    \midrule % Vanilla Cascading
         Vanilla & & & & & & & Part-Of-Speech (POS)/Chunking/Combinatory & & &  \\
         
         % (Short Paper)
         Cascading & \multirow{-2}{*}{ACL} & \multirow{-2}{*}{\citeyear{sogaard-goldberg-2016-deep}} & \multirow{-2}{*}{Cascading} & \multirow{-2}{*}{LSTM} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Text} & Categorical Grammar (CCG) Supertagging & \multirow{-2}{*}{F1 score, Micro-F1 score} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{---}\\

    \rowcolor{gray!20}
    \midrule % Cross-stitch
         &  &  & & & & & Surface normals estimation (normals)/semantic & mErr/median error (medErr)/within $t^{\circ}$ in angular & & \\
    \rowcolor{gray!20}
        \multirow{-1.8}{*}{Cross-stitch} & & & & & & & segmentation (semseg), object detection/attribute & distance (within $t^{\circ}$), pixel accuracy (pixacc), & & \\
    \rowcolor{gray!20}
        \multirow{-1.8}{*}{networks} & \multirow{-3}{*}{CVPR} & \multirow{-3}{*}{\citeyear{misra2016cross}} & \multirow{-3}{*}{---} & \multirow{-3}{*}{CNN} & \multirow{-3}{*}{Soft} & \multirow{-3}{*}{Image} & prediction & mIoU, fwIU, mAP & \multirow{-3}{*}{CE loss} & \multirow{-3}{*}{\href{https://github.com/helloyide/Cross-stitch-Networks-for-Multi-task-Learning}{\textcolor{reforange}{Unofficial}}} \\
        

    \midrule % ASP-MTL
    % \rowcolor{gray!20}
        ASP-MTL (aka & & & & & Hard \& & & & & CE loss, adversarial loss, & \\
    % \rowcolor{gray!20}
       AdvMTL) & \multirow{-2}{*}{arXiv} & \multirow{-2}{*}{\citeyear{liu2017adversarial}} & \multirow{-2}{*}{Adversarial training} & \multirow{-2}{*}{LSTM} & Soft & \multirow{-2}{*}{Text} & \multirow{-2}{*}{Text classifications} & \multirow{-2}{*}{Error rate} & orthogonality constraint & \multirow{-2}{*}{\href{http://pfliu.com/paper/adv-mtl.html}{\textcolor{citegreen}{Official}}}\\


    \midrule % JMT
    \rowcolor{gray!20}
        & & & Cascading, adding & & & & Part-Of-Speech (POS) tagging/chunking/parsing/ & Accuracy (acc), F1, MSE, unlabeled attachment & CE loss, softmax loss, & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{JMT} & \multirow{-2}{*}{EMNLP} & \multirow{-2}{*}{\citeyear{hashimoto-jmt:2017:EMNLP2017}} & constraints & \multirow{-2}{*}{LSTM} & \multirow{-2}{*}{Soft} & \multirow{-2}{*}{Text} & semantic relatedness/textual entailment & score (UAS)/labeled attachment score (LAS) & KL-divergence & \multirow{-2}{*}{\href{https://github.com/rubythonode/joint-many-task-model}{\textcolor{reforange}{Unofficial}}}\\
        
    \midrule % MNCs
    % \rowcolor{gray!20}
        & & & & & & & Object detection/mask estimation/object  & & RPN loss~\citep{ren2015faster}, & \\
    % \rowcolor{gray!20}
        \multirow{-2}{*}{MNCs} & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{dai2016instance}} & \multirow{-2}{*}{Cascading} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & categorization & \multirow{-2}{*}{mAP$@$IoU} & mask regression loss, softmax loss & \multirow{-2}{*}{\href{https://github.com/daijifeng001/MNC}{\textcolor{citegreen}{Official}}}\\
    


    % \midrule % PathNet
    %     \multirow{2}{*}{PathNet~\citeyear{fernando2017pathnet}} & \multirow{2}{*}{arXiv} & \multirow{2}{*}{2017} & \multirow{2}{*}{NAS, transfer learning} & CNN & \multirow{2}{*}{Adaptive} & \multirow{2}{*}{Image, state} & \multirow{2}{*}{classification, Atari/Labyrinth game} & \multirow{2}{*}{Acc, AUC} & \multirow{2}{*}{CE loss} & \multirow{2}{*}{\href{https://github.com/kimhc6028/pathnet-pytorch}{\textcolor{citegreen}{Official}}}\\
        
    %      & & & & & & & & & & \\

    \midrule % FAFS
    \rowcolor{gray!20}
        FAFS & CVPR & \citeyear{lu2017fully} & NAS & CNN & Hard & Image & person attribute classification & Acc/recall & CE loss &\href{https://github.com/luyongxi/deep_share}{\textcolor{citegreen}{Official}} \\

                
    \midrule % MRN
    % \rowcolor{gray!20}
        & & & & & Hard \& & & & & & \\
    % \rowcolor{gray!20}
        \multirow{-2}{*}{MRN} & \multirow{-2}{*}{NeurIPS} & \multirow{-2}{*}{\citeyear{long2017learning}} & \multirow{-2}{*}{Task conditioning} & \multirow{-2}{*}{CNN} & Soft & \multirow{-2}{*}{Image} & \multirow{-2}{*}{classifications on different domains} & \multirow{-2}{*}{Acc} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{\href{https://github.com/thuml/MTlearn}{\textcolor{citegreen}{Official}}}\\


    % \midrule % gradnorm
    %     \multirow{2}{*}{GradNorm~\citeyear{chen2018gradnorm}} & \multirow{2}{*}{ICML} & \multirow{2}{*}{2018} & \multirow{2}{*}{task balancing} & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & Semseg/depth/normals/keypoints & \multirow{2}{*}{RMSE, IoU, 1 $-$ cosine similarity (cos), mErr} & CE loss, $\ell_1$ loss, $\ell_2$ loss & \multirow{2}{*}{\href{https://github.com/hosseinshn/GradNorm}{\textcolor{reforange}{Unofficial}}}\\
        
    %     & & & & & & & prediction (keypoints) & & cosine loss & \\

    % \midrule % uncertainty weighting
    %     Uncertainty & \multirow{2}{*}{CVPR} & \multirow{2}{*}{2018} & \multirow{2}{*}{Task balancing} & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & \multirow{2}{*}{Semseg/depth/classification} & \multirow{2}{*}{IoU, mErr/RMSE} & CE loss, $\ell_1$ loss, uncertainty & \multirow{2}{*}{\href{https://github.com/yaringal/multi-task-learning-example}{\textcolor{citegreen}{Official}}}\\
        
    %     Weighting~\citeyear{kendall2018multi} & & & & & & & & & loss~\citeyear{kendall2018multi} & \\

    \midrule % PAD-Net
    \rowcolor{gray!20}
        &  &  &  &  &  &  & Depth/scene parsing/contour & & CE loss, softmax loss & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{PAD-Net} & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{xu2018pad}} & \multirow{-2}{*}{Mutual distillation} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & prediction/normals & \multirow{-2}{*}{rel/RMSE/log10 mErr/acc-$\delta$, IoU/acc} & Euclidean loss & \multirow{-2}{*}{---}\\

    \midrule % MTAN
        MT$\text{A}_{(\text{adv})}$N & CVPR & \citeyear{liu2018multi} & Adversarial training & CNN & Hard & Image & font/glyph, identity/pose/illumination & Recognition rate & CE loss, adversarial loss & ---\\
        
        

    \midrule % TRL
    \rowcolor{gray!20}
        & & & cross-task & & & & & Mean relative error (rel)~\citep{eigen2014depth}/RMSE/ & berHu loss~\citep{laina2016deeper}, & \\ % liu2015deep
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{TRL} & \multirow{-2}{*}{ECCV} & \multirow{-2}{*}{\citeyear{zhang2018joint}} & attention & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & \multirow{-2}{*}{Depth estimation (depth)/semseg} & acc with threshold $\delta$ (acc-$\delta$), pixacc/mean acc/mIoU & CE loss, uncertainty loss & \multirow{-2}{*}{---}\\



                
    % \midrule % MGDA-MTL
    %     MGDA- & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{2018} & \multirow{2}{*}{task balancing} & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & classification/regression, semseg/instance & \multirow{2}{*}{mErr, disparity error} & \multirow{2}{*}{CE loss, $\ell_1$ loss, RMSE} & \multirow{2}{*}{\href{https://github.com/isl-org/MultiObjectiveOptimization}{\textcolor{citegreen}{Official}}}\\

    %     MTL~\citeyear{sener2018multi} & & & & & & & segmentation (instance)/depth & & & \\

    \midrule % MMoE
        \multirow{2}{*}{MMoE} & \multirow{2}{*}{KDD} & \multirow{2}{*}{\citeyear{ma2018modeling}} & MoE & \multirow{2}{*}{MLP} & Hard \& & Tabular & Income/education/marriage prediction,  & \multirow{2}{*}{Area Under the Curve (AUC)} & \multirow{2}{*}{CE loss} & \multirow{2}{*}{\href{https://github.com/shenweichen/DeepCTR}{\textcolor{reforange}{Unofficial}}}\\
        
        & & & & & soft & data & engagement/satisfaction in recommendation & & & \\
       % https://github.com/shenweichen/DeepCTR-Torch
       % https://github.com/shenweichen/DeepCTR

    \midrule % Soft Order
    \rowcolor{gray!20}
        & & & & & & Tabular & & & & \\
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{Soft Order} & \multirow{-2}{*}{ICLR} & \multirow{-2}{*}{\citeyear{meyerson2018beyond}} & \multirow{-2}{*}{feature fusion} & \multirow{-2}{*}{CNN, MLP} & \multirow{-2}{*}{Soft} & data, image & \multirow{-2}{*}{Classification, attribute recognition}  & \multirow{-2}{*}{mErr} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{---}\\

    \midrule % GREAT4MTL
    % \rowcolor{gray!20}
         & & & & & &  & classification/colorization/edge/denoised & & & \\
        
    % \rowcolor{gray!20}
        \multirow{-2}{*}{GREAT4MTL} & \multirow{-2}{*}{arXiv} & \multirow{-2}{*}{\citeyear{sinha2018gradient}} & \multirow{-2}{*}{adversarial training} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & reconstruction, depth/normal/keypoint & \multirow{-2}{*}{Err, RMSE, $1 - |\text{cos}(\cdot, \cdot)|$} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{---}\\


    \midrule % Sluice networks
    \rowcolor{gray!20}
        Sluice &  &  & Adding constraints, &  & Hard \& &  &  Chunking/entity recognition (NER)/semantic  &  &  & \\
    \rowcolor{gray!20}
        networks & \multirow{-2}{*}{AAAI} & \multirow{-2}{*}{\citeyear{ruder2019latent}} & early stopping  & \multirow{-2}{*}{LSTM} & Soft & \multirow{-2}{*}{Text} & role labeling (SRL)/POS tagging & \multirow{-2}{*}{Acc} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{\href{https://github.com/sebastianruder/sluice-networks}{\textcolor{citegreen}{Official}}} \\

        
    \midrule % Hierarchical MTL
    % \rowcolor{gray!20}
         & & & & CNN, & & & NER/Entity Mention Detection (EMD)/Relation & F1 score/precision/recall, MUC/B3/CEAFe & & \\
    % \rowcolor{gray!20}
         \multirow{-2}{*}{HMTL} & \multirow{-2}{*}{AAAI} & \multirow{-2}{*}{\citeyear{sanh2019hierarchical}} & \multirow{-2}{*}{cascading} & LSTM & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Text} & Extraction (RE)/Coreference Resolution (CR) & \citep{moosavi2016coreference} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{\href{https://github.com/huggingface/hmtl}{\textcolor{reforange}{Unofficial}}} \\

         
    \midrule % Deep Cascade Multi-Task Learning
    \rowcolor{gray!20}
         & & & & CNN, & & & Segment labeling/Named Entity Labeling & & CRF loss~\citep{xu2013convolutional}, CE& \\
    \rowcolor{gray!20}    
         \multirow{-2}{*}{DCMTL} & \multirow{-2}{*}{AAAI} & \multirow{-2}{*}{\citeyear{gong2019deep}} & \multirow{-2}{*}{cascading} & LSTM & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Text} & (NEL)/slot filling & \multirow{-2}{*}{F1 score/precision/recall} & loss, ranking loss~\citep{vu2016bi} & \multirow{-2}{*}{\href{https://github.com/gy910210/DCMTL}{\textcolor{citegreen}{Official}}} \\

        
    \midrule % nddr-cnn
    % \rowcolor{gray!20}
         & & & & & & & Normals/semseg, age estimation/gender & mErr/medErr/within $t^{\circ}$, mIoU, pixacc, mean/ & & \\
    % \rowcolor{gray!20}
         \multirow{-2}{*}{NDDR-CNN} & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{gao2019nddr}} & \multirow{-2}{*}{feature fusion} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Soft} & \multirow{-2}{*}{Image} & classification & median absolute error (absErr), acc & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{\href{https://github.com/ethanygao/NDDR-CNN}{\textcolor{citegreen}{Official}}} \\


    \midrule % PAP
    \rowcolor{gray!20}
        &  &  & cross-task &  &  &  &  & RMSE/rel/acc with $t$, mErr/medError/within & CE loss, $\ell_1$ loss, Pair-wise affinity & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{PAP} & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{zhang2019pattern}} & attention & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & \multirow{-2}{*}{Semseg/depth/normals} & $t^{\circ}$, mIoU/mean accuracy (mAcc)/pixacc & loss~\citep{zhang2019pattern}, berHu loss  & \multirow{-2}{*}{---} \\

        
    \midrule % MTAN
    % \rowcolor{gray!20}
        MT$\text{A}_{(\text{atten})}$N & & & & & Hard \& & & Semseg/depth/normals, 10 classifications & mIoU/pixacc, mErr/medErr/within $t^{\circ}$, & &  \\ 

    % \rowcolor{gray!20}
        (\& DWA) & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{liu2019end}} & \multirow{-2}{*}{Adaptive weighting} & \multirow{-2}{*}{CNN} & Soft & \multirow{-2}{*}{Image} & (visual domain decathlon\tnote{2}\,\,\,) & absErr/real error, accuracy & \multirow{-2}{*}{CE loss, $\ell_1$ loss, dot product} & \multirow{-2}{*}{\href{https://github.com/lorenmt/mtan}{\textcolor{citegreen}{Official}}} \\ 

    
    % \midrule % MultiNet++
    %     \multirow{2}{*}{MultiNet++~\citeyear{chennupati2019multinet++}} & CVPR & \multirow{2}{*}{2019} & geometric loss & \multirow{2}{*}{CNN} & Hard \& & \multirow{2}{*}{Video} & \multirow{2}{*}{Semseg/depth/moving object detection} & \multirow{2}{*}{Acc} & geometric mean of CE & \multirow{2}{*}{---} \\
        
    %     & Workshop & & strategy~\citeyear{chennupati2019multinet++} & & Soft & & & & loss and Huber loss~\citeyear{huber1964robust} & \\

    \midrule % ASTMT
    \rowcolor{gray!20}
        & & & & & & & Semseg/depth/edge/normals/human parts/ & mIoU/osdF/mErr/maximum F-measure (maxF)/ &  & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{ASTMT} & \multirow{-2}{*}{CVPR} & \multirow{-2}{*}{\citeyear{maninis2019attentive}} & \multirow{-2}{*}{attention, single-tasking} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & saliency estimation/albedo & RMSE/$\Delta_m$ & \multirow{-2}{*}{CE loss, $\ell_1$ loss} & \multirow{-2}{*}{\href{https://github.com/facebookresearch/astmt}{\textcolor{citegreen}{Official}}}\\

    \midrule % ML-GCN
    % \rowcolor{gray!20}
        {ML-GCN} & CVPR & \citeyear{chen2019multi} & Graph based & CNN, GCN & Hard & Image & Multi-label recognition & precision, recall, F1 & CE loss & \href{https://github.com/megvii-research/ML-GCN}{\textcolor{citegreen}{Official}} \\

    \midrule % RD4MTL
    \rowcolor{gray!20}
        RD4MTL & arXiv & \citeyear{meng2019representation} & Adversarial training & CNN & Hard & Image & Classifications & Acc & CE loss, adversarial loss & \href{https://github.com/qmeng99/Multi-task-Representation-Disentanglement}{\textcolor{citegreen}{Official}} \\

    \midrule % MTL-NAS
        \multirow{2}{*}{MTL-NAS} & \multirow{2}{*}{CVPR} & \multirow{2}{*}{\citeyear{gao2020mtl}} & \multirow{2}{*}{NAS} & \multirow{2}{*}{CNN} & \multirow{2}{*}{---} & \multirow{2}{*}{Image} & Semseg/normals, object classification/scene & mErr/medErr/Within $t^\circ$, mIoU/pixacc, & CE loss, $\ell_2$ loss, minimum entropy & \multirow{2}{*}{\href{https://github.com/bhpfelix/MTLNAS}{\textcolor{citegreen}{Official}}}\\

        & & & & & & & classification & Acc & regularization~\citep{gao2020mtl} & \\
        
    \midrule % BMTN
    \rowcolor{gray!20}
         & & & & & & & Semseg/edge/depth/keypoint detection (point), & & & \\
    \rowcolor{gray!20} % DBLP:conf/bmvc/VandenhendeGGB20
         \multirow{-2}{*}{BMTN} & \multirow{-2}{*}{BMVC} & \multirow{-2}{*}{\citeyear{vandenhende2019branched}} & \multirow{-2}{*}{NAS} & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{---} & \multirow{-2}{*}{Image} & attribute classification &  \multirow{-2}{*}{mIoU, pixacc, $\ell_1$, Acc} & \multirow{-2}{*}{CE loss, $\ell_1$ loss, $\Delta_m$} & \multirow{-2}{*}{\href{https://github.com/hurricane2018/Branched-Multi-Task-Networks-Deciding-What-Layers-To-Share}{\textcolor{citegreen}{Official}}}\\
    

        
    \midrule % PSD
        \multirow{2}{*}{PSD} & \multirow{2}{*}{CVPR} & \multirow{2}{*}{\citeyear{zhou2020pattern}} & \multirow{2}{*}{Distillation}& \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard \& soft} & \multirow{2}{*}{Image} & \multirow{2}{*}{Semseg/depth/normals} & RMSE/rel/acc with $t$, mIoU/mean accuracy/ & \multirow{2}{*}{CE loss, $\ell_1$ loss, berHu loss} & \multirow{2}{*}{---}\\

        & & & & & & & & pixacc, mErr/medErr/within $t^{\circ}$  & & \\

    \midrule % KD4MTL
    \rowcolor{gray!20}
        & ECCV & & distillation & & Hard \& & & & mIoU/pixacc, absErr/rel, mErr/medErr/within & & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{KD4MTL} & Workshop & \multirow{-2}{*}{\citeyear{li2020knowledge}} & knowledge & \multirow{-2}{*}{CNN} & soft & \multirow{-2}{*}{Image} & \multirow{-2}{*}{Semseg/depth/normals, classification} & $t^\circ$, Acc & \multirow{-2}{*}{CE loss, $\ell_1$ loss, dot product} & \multirow{-2}{*}{\href{https://github.com/VICO-UoE/KD4MTL}{\textcolor{citegreen}{Official}}} \\
    
        
    \midrule % MTI-Net
        \multirow{2}{*}{MTI-Net} & \multirow{2}{*}{ECCV} & \multirow{2}{*}{\citeyear{vandenhende2020mti}} & multi-task & \multirow{2}{*}{CNN} & Hard \& & \multirow{2}{*}{Image} & Semseg/depth/edges detection (edges)/normals/ & mIoU, RMSE, mErr, optimal dataset-scale F- & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{\href{https://github.com/SimonVandenhende/Multi-Task-Learning-PyTorch}{\textcolor{citegreen}{Official}}}\\

        & & & distillation & & Soft & & saliency estimation/human parts  & measure (odsF)~\citep{martin2004learning}, $\Delta_m$ & & \\

    \midrule % LTB
    \rowcolor{gray!20}
        & & & NAS, & & & & Regression, face attribute prediction, semseg/ & & & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{LTB} & \multirow{-2}{*}{ICML} & \multirow{-2}{*}{\citeyear{guo2020learning}} & task grouping & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Soft} & \multirow{-2}{*}{Image} & normals/depth/keypoints/edges & \multirow{-2}{*}{Acc, CE, cos, mean absErr}  & \multirow{-2}{*}{CE loss, $\ell_1$ loss, cosine loss} & \multirow{-2}{*}{---} \\

    \midrule % AAMTRL: Adaptive Adversarial Multi-task Representation Learning
    % \rowcolor{gray!20}
        & & & & CNN \& & & &  & & & \\
    % \rowcolor{gray!20}
        \multirow{-2}{*}{AAMTRL} & \multirow{-2}{*}{ICML} & \multirow{-2}{*}{\citeyear{mao2020adaptive}} & \multirow{-2}{*}{adversarial training} & LSTM & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Text} & \multirow{-2}{*}{Classifications} & \multirow{-2}{*}{Relatedness evolution, acc, influence of \#task}  & \multirow{-2}{*}{Any 1-Lipschitz loss} & \multirow{-2}{*}{---} \\
    


    % \midrule % PCGrad
    %     \multirow{2}{*}{PCGrad~\citeyear{yu2020gradient}} & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{2020} & \multirow{2}{*}{task balancing} & CNN \& & Hard \& & Image, & Semseg/depth/normals, classification, face & mIoU/pixacc, absErr/rel, mErr/medErr/within & \multirow{2}{*}{CE loss, $\ell_1$ loss, $\ell_2$ loss} & \multirow{2}{*}{\href{https://github.com/tianheyu927/PCGrad}{\textcolor{citegreen}{Official}}}\\
        
    %     & & & & SAC & Soft & state\tnote{3} & attribute prediction, robot action prediction & $t^\circ$, Acc/mErr, success rate & & \\

    % \midrule % GradDrop
    %     \multirow{2}{*}{GradDrop~\citeyear{chen2020just}} & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{2020} & \multirow{2}{*}{Task balancing} & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & Image, & attribute prediction, classification, coordinate/ & mErr, F1, Average Precision score (AP)/ & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{\href{https://github.com/tensorflow/lingvo/blob/master/lingvo/core/graddrop.py}{\textcolor{citegreen}{Official}}}\\
        
    %     & & & & & & LiDAR & dimension/orientation/class in object detection & Average Precision w/ Heading (APH) score & & \\

    % \midrule % Adashare
    %     \multirow{2}{*}{Adashare} & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{\citeyear{sun2020adashare}} & \multirow{2}{*}{NAS} & \multirow{2}{*}{---} & \multirow{2}{*}{---} & Tabular &  & & \multirow{2}{*}{---} & \multirow{2}{*}{\href{https://github.com/shenweichen/DeepCTR}{\textcolor{reforange}{Unofficial}}}\\
        
    %     & & & & & & & & & & \\

    \midrule % CGC & PLE
    \rowcolor{gray!20}
        & & & & & Hard \& & Tabular & Sub-tasks in the recommendation systems, & & & \\
    \rowcolor{gray!20} % (Best Paper)
        \multirow{-2}{*}{CGC \& PLE} & \multirow{-2}{*}{RecSys} & \multirow{-2}{*}{\citeyear{tang2020progressive}} & \multirow{-2}{*}{} & \multirow{-2}{*}{MLP} & soft & data & income/education/marriage prediction & \multirow{-2}{*}{AUC/MSE, MTL gain} & \multirow{-2}{*}{CE loss, $\ell_2$ loss} & \multirow{-2}{*}{\href{https://github.com/shenweichen/DeepCTR}{\textcolor{reforange}{Unofficial}}}\\
    

    % \midrule % AuxiLearn
    %     \multirow{2}{*}{AuxiLearn~\citeyear{navon2021auxiliary}} & \multirow{2}{*}{ICLR} & \multirow{2}{*}{2021} & \multirow{2}{*}{Task balancing} & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & classification/auxiliary tasks, Semseg/depth/  & \multirow{2}{*}{Acc, mIoU/pixacc} & CE loss, $\ell_1$ loss, dot product, & \multirow{2}{*}{\href{https://github.com/AvivNavon/AuxiLearn}{\textcolor{citegreen}{Official}}}\\
        
        
        % & & & & & & & normals & & auxiliary loss~\citeyear{navon2021auxiliary} & \\

    % \midrule % IMTL
    %     \multirow{2}{*}{IMTL~\citeyear{liu2021towards}} & \multirow{2}{*}{ICLR} & \multirow{2}{*}{2021} & task & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & Semseg/instsance/disparity estimation & \multirow{2}{*}{mIoU, $\ell_1$, cos, acc} & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{\href{https://github.com/JohnLaMaster/Impartial-Multi-Task-Learning}{\textcolor{reforange}{Unofficial}}}\\
        
        
    %     & & & balancing & & & & (disparity)/normals/depth, classification & & & \\

    %     \midrule % GradVac
    %     \multirow{2}{*}{GradVac~\citeyear{wang2021gradient}} & \multirow{2}{*}{ICLR} & \multirow{2}{*}{2021} & task & \multirow{2}{*}{Transformer} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Text} & Multilingual Machine Translation, multilingual & \multirow{2}{*}{BLEU score~\citeyear{10.3115/1073083.1073135}, F1} & \multirow{2}{*}{CE loss} & \multirow{2}{*}{\href{https://github.com/chenllliang/Gradient-Vaccine}{\textcolor{reforange}{Unofficial}}}\\
        
    %     & & & balancing & & & & NER, multilingual POS & & & \\

    \midrule % TSNs
        \multirow{2}{*}{TSNs} & \multirow{2}{*}{ICCV} & \multirow{2}{*}{\citeyear{sun2021task}} & task relationship learning, & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & Semseg/depth/edges/normals/ & \multirow{2}{*}{mIoU, RMSE, mErr, odsF, $\Delta_m$} & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{\href{https://github.com/GuoleiSun/TSNs}{\textcolor{citegreen}{Official}}}\\

        & & & task conditioning & & & & saliency estimation/human parts & & & \\

    \midrule % MuST
    \rowcolor{gray!20}
        & & & knowledge distillation, & & & & Classification/detection/semseg/depth/ & & & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{MuST} & \multirow{-2}{*}{ICCV} & \multirow{-2}{*}{\citeyear{ghiasi2021multi}} & task conditioning & \multirow{-2}{*}{CNN} & \multirow{-2}{*}{Hard} & \multirow{-2}{*}{Image} & normals & \multirow{-2}{*}{Acc, mIoU, RMSE, odsF} & \multirow{-2}{*}{CE loss, $\ell_1$ loss} & \multirow{-2}{*}{---}\\ % metric may be wrong



    \midrule % AuxSegNet
        \multirow{2}{*}{AuxSegNet} & \multirow{2}{*}{ICCV} & \multirow{2}{*}{\citeyear{xu2021leveraging}} & cross-task & \multirow{2}{*}{CNN} & Hard \& & \multirow{2}{*}{Image} & \multirow{2}{*}{Semseg/classification/saliency detection} & \multirow{2}{*}{mIoU/precision/recall} & Multi-label softmax & \multirow{2}{*}{\href{https://github.com/xulianuwa/AuxSegNet}{\textcolor{citegreen}{Official}}}\\
        
        & & & attention  & & Soft & & & & loss, CE loss& \\

    \midrule % ATRC module
    \rowcolor{gray!20}
        & & & cross-task & & Hard \& & & Semseg/depth estimation/edges/normals/ & & & \\
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{ATRC} & \multirow{-2}{*}{ICCV} & \multirow{-2}{*}{\citeyear{bruggemann2021exploring}} & attention & \multirow{-2}{*}{CNN} & soft & \multirow{-2}{*}{Image} & saliency estimation/human parts & \multirow{-2}{*}{mIoU, RMSE, mErr, odsF, maxF, $\Delta_m$} & \multirow{-2}{*}{CE loss, $\ell_1$ loss} & \multirow{-2}{*}{\href{https://github.com/brdav/atrc}{\textcolor{citegreen}{Official}}}\\

    

                
    % \midrule % CAGrad
    %     \multirow{2}{*}{CAGrad~\citeyear{liu2021conflictaverse}} & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{2021} & task & \multirow{2}{*}{CNN, SAC} & Hard \& & Image & Semseg/depth/normals, robot action prediction,& mIoU/pixacc, mErr/medErr/within $t^\circ$, absErr/ & \multirow{2}{*}{CE loss, $\ell_1$ loss, dot product} & \multirow{2}{*}{\href{https://github.com/Cranial-XIX/CAGrad}{\textcolor{citegreen}{Official}}}\\
        
    %     & & & balancing & & Soft & state & classification & rel, $\Delta m$ &  & \\

    \midrule % DSelect-k
        \multirow{2}{*}{DSelect-k} & \multirow{2}{*}{NeurIPS} & \multirow{2}{*}{\citeyear{hazimeh2021dselect}} & \multirow{2}{*}{MoE} & \multirow{2}{*}{MLP, CNN} & Hard \& & Tabular & \multirow{2}{*}{engagement/satisfaction task, classification} & \multirow{2}{*}{Total loss, Acc, AUC/RMSE, \#expert}  & \multirow{2}{*}{CE loss, $\ell_2$ loss} & \multirow{2}{*}{\href{https://github.com/google-research/google-research/tree/master/dselect_k_moe}{\textcolor{citegreen}{Official}}}\\
        
        & & & & & soft & data, Image &  &  & & \\

    \midrule % MT-TaG
    \rowcolor{gray!20}
        & & & & & Hard \& & & 16 Language understanding tasks, e.g. textual & Acc, Spearman correlation~\citeyear{spearman1961proof}, Matthews & & \\
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{MT-TaG} & \multirow{-2}{*}{ArXiv} & \multirow{-2}{*}{\citeyear{gupta2022sparsely}} & \multirow{-2}{*}{MoE} & \multirow{-2}{*}{Transformer} & soft & \multirow{-2}{*}{Text} & entailment, sentiment classification, etc. & correlation coefficient~\citep{matthews1975comparison}  & \multirow{-2}{*}{CE loss, MSE} & \multirow{-2}{*}{---}\\

    \midrule % CrossDistil
    \rowcolor{gray!20}
        & & & & & Hard \& & Tabular & &  & & \\
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{CrossDistil} & \multirow{-2}{*}{AAAI} & \multirow{-2}{*}{\citeyear{yang2022cross}} & \multirow{-2}{*}{distillation} & \multirow{-2}{*}{MLP} & soft & data & \multirow{-2}{*}{Finish watching/like} & \multirow{-2}{*}{AUC, multi-AUC~\citep{hand2001simple}}  & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{---}\\


    % \midrule % RLW & RGW
    %     RLW \& RGW & \multirow{2}{*}{TMLR} & \multirow{2}{*}{2022} & task & CNN, & Hard \& & Image, & Classification, semseg/depth/normals, & Acc, F1, $\Delta_p$, gradient flatness, mIoU/pixacc, & \multirow{2}{*}{CE loss, $\ell_1$ loss, cosine loss} & \multirow{2}{*}{\href{https://github.com/median-research-group/libmtl}{\textcolor{reforange}{Unofficial}}}\\
        
    %     \citeyear{lin2022reasonable} & & & balancing & Transformer & Soft & Text & multilingual paraphrase identification (PI)/POS & absErr/rel, mErr/medErr/within $t^\circ$ & & \\

    \midrule % MulT
        \multirow{2}{*}{MulT} & \multirow{2}{*}{CVPR} & \multirow{2}{*}{\citeyear{bhattacharjee2022mult}} & cross-task & CNN \& & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & Semseg/depth/reshading/normals/ & MTL gain, mErr of & CE loss, $\ell_1$ loss, & \multirow{2}{*}{\href{https://ivrl.github.io/MulT/}{\textcolor{citegreen}{Official}}}\\
        
        & & & attention & Transformer & & & keypoints/edges & domain generalization & rotate loss~\citep{zamir2018taskonomy} & \\

    \midrule % MTFormer

    \rowcolor{gray!20}
        & & & cross-task attention, & & & & & & CE loss, $\ell_1$ loss, cross- & \\

    \rowcolor{gray!20}
        & & & task balancing (\textit{spec.}, & & \multirow{-1.8}{*}{Hard \&} & & \multirow{-1.8}{*}{Semseg/depth/saliency detection/} & & task contrastive loss, & \\
        
    \rowcolor{gray!20}
        \multirow{-3}{*}{MTFormer} & \multirow{-3}{*}{ECCV} & \multirow{-3}{*}{\citeyear{xu2022mtformer}} & \citet{kendall2018multi}) & \multirow{-3}{*}{Transformer} & \multirow{-1.8}{*}{soft} & \multirow{-3}{*}{Image} & \multirow{-1.8}{*}{human parts} & \multirow{-3}{*}{mIoU, RMSE, $\Delta_m$} & uncertainty loss & \multirow{-3}{*}{---}\\

    \midrule % MQTransformer
        \multirow{2}{*}{MQTransformer} & \multirow{2}{*}{arXiv} & \multirow{2}{*}{\citeyear{xu2022multi}} & cross-task & \multirow{2}{*}{Transformer} & Hard \& & \multirow{2}{*}{Image} & Semseg/depth/edges/normals/saliency & \multirow{2}{*}{mIoU, RMSE, mErr, odsF, maxF} & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{---}\\
        
        & & & attention & & Soft & &  estimation/human parts & & & \\

    % \midrule % Nash-MTL
    %     \multirow{2}{*}{Nash-MTL~\citeyear{navon2022multi}} & \multirow{2}{*}{ICML} & \multirow{2}{*}{2022} & \multirow{2}{*}{Task balancing} & CNN, GRU, & \multirow{2}{*}{\jun{Hard/Soft}} & Image & Semseg/depth/normals, regression, robot & Pixacc/mIoU, absErr/rel, mErr/medErr/within & CE loss, $\ell_1$ loss, dot product, & \multirow{2}{*}{\href{https://github.com/AvivNavon/nash-mtl}{\textcolor{citegreen}{Official}}}\\
    %     % Check MTL methods in the link below
    %     % https://github.com/AvivNavon/nash-mtl
    %     & & & & \& SAC~\citeyear{haarnoja2018soft} & & graph, state & action prediction  & $t^\circ$, success rate, mean rank\tnote{4}~~~, $\Delta_m$ & $\ell_2$ loss, Nash Bargaining term & \\

    % \midrule % Rotagrad
    %     \multirow{2}{*}{Rotograd~\citeyear{javaloy2022rotograd}} & \multirow{2}{*}{ICLR} & \multirow{2}{*}{2022} & task & \multirow{2}{*}{CNN} & \multirow{2}{*}{Hard} & \multirow{2}{*}{Image} & \multirow{2}{*}{Classification, semseg/depth/normals} & $\Delta_m$, F1, mIoU/pixacc, absErr/rel, mErr/medErr/ & \multirow{2}{*}{CE loss} & \multirow{2}{*}{\href{https://github.com/adrianjav/rotograd}{\textcolor{citegreen}{Official}}}\\
        
    %     & & & balancing & & & & & within $t^\circ$ & & \\

    \midrule % MetaLink
    \rowcolor{gray!20}
        & & & & & & Image, & & & & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{MetaLink} & \multirow{-2}{*}{ICLR} & \multirow{-2}{*}{\citeyear{cao2022relational}} & \multirow{-2}{*}{Graph based} & \multirow{-2}{*}{MLP, GNN} & \multirow{-2}{*}{Hard} & Graph & \multirow{-2}{*}{Classification} & \multirow{-2}{*}{mAP, ROC AUC} & \multirow{-2}{*}{CE loss} & \multirow{-2}{*}{\href{https://github.com/snap-stanford/GraphGym}{\textcolor{citegreen}{Official}}}\\ 
        % code link is strange
    

    \midrule % DeMT
        \multirow{2}{*}{DeMT} & \multirow{2}{*}{AAAI} & \multirow{2}{*}{\citeyear{zhang2023demt}} & cross-task & \multirow{1}{*}{CNN \&} & Hard \& & \multirow{2}{*}{Image} & Semseg/depth/edges/normals/saliency  & \multirow{1}{*}{mIoU, RMSE, mErr, odsF, maxF,} & \multirow{2}{*}{CE loss, $\ell_1$ loss} & \multirow{2}{*}{\href{https://github.com/yangyangxu0/DeMT}{\textcolor{citegreen}{Official}}} \\
        
        & & & attention & \multirow{1}{*}{Transformer} & Soft & & estimation/human parts & \multirow{1}{*}{$\Delta_m$} & &  \\

    \midrule % mTEB
    \rowcolor{gray!20}
        & & & cross-task & & Hard \& & & & & CE loss, berHu loss, cosine & \\
    \rowcolor{gray!20}
        \multirow{-2}{*}{mTEB} & \multirow{-2}{*}{WACV} & \multirow{-2}{*}{\citeyear{lopes2023cross}} & attention & \multirow{-2}{*}{CNN} & soft & \multirow{-2}{*}{Image} & \multirow{-2}{*}{Semseg/depth/normals/edges} & \multirow{-2}{*}{$\Delta_m$, mIoU, RMSE, mErr, F1} & loss~\citep{guizilini2021geometric} & \multirow{-2}{*}{\href{https://github.com/astra-vision/DenseMTL}{\textcolor{citegreen}{Official}}}\\



    \midrule % OKD-MTL
        \multirow{2}{*}{OKD-MTL} & \multirow{2}{*}{WACV} & \multirow{2}{*}{\citeyear{jacob2023online}} & distillation, task & \multirow{2}{*}{Transformer} & Hard \& & \multirow{2}{*}{Image} & \multirow{2}{*}{Semseg/depth/normals} & $\Delta_p$, mIoU/pixacc, absErr/rel, mErr/medErr/ & Adaptive feature distillation loss, & \multirow{2}{*}{---}\\
        
        & & & weighting & & Soft & & & within $t^\circ$ & CE loss, $\ell_1$ loss, cosine loss & \\

    \midrule % AdaMV-MoE
    \rowcolor{gray!20}
        & & & & & Hard \& & & & & & \\
        
    \rowcolor{gray!20}
        \multirow{-2}{*}{AdaMV-MoE} & \multirow{-2}{*}{ICCV} & \multirow{-2}{*}{\citeyear{chen2023adamv}} & \multirow{-2}{*}{MoE} & \multirow{-2}{*}{Transformer} & soft & \multirow{-2}{*}{Image} & \multirow{-2}{*}{classification/detection/Seg} & \multirow{-2}{*}{Acc, Average Precision (AP)} & \multirow{-2}{*}{CE loss}& \multirow{-2}{*}{\href{https://github.com/google-research/google-research/tree/master/moe_mtl}{\textcolor{citegreen}{Official}}}\\

    % \midrule % moco
    %     \multirow{2}{*}{MoCo~\citeyear{fernando2023mitigating}} & \multirow{2}{*}{ICLR } & \multirow{2}{*}{2023} & task & \multirow{2}{*}{CNN, SAC} & \multirow{2}{*}{Hard} & Image, & Semseg/depth/normals, robot action & mIoU/pixacc, absErr/rel, mErr/medErr/within & \multirow{2}{*}{CE loss, $\ell_1$ loss, $\ell_2$ loss} & \multirow{2}{*}{---}\\
        
    %     & & & balancing & & & state &  prediction, classification & $t^\circ$, success rate, Acc, $\Delta_m$ & & \\

    % \midrule % Recon
    % \rowcolor{gray!20}
    %     & & & MTL Strategy 2 & & & & task 2  & measure 2 & & \\
        
    % \rowcolor{gray!20}
    %     \multirow{-2}{*}{Recon~\citeyear{shi2023recon}} & \multirow{-2}{*}{ICLR} & \multirow{-2}{*}{2023} & MTL Strategy 1 & \multirow{-2}{*}{Backbone} & \multirow{-2}{*}{H/S} & \multirow{-2}{*}{Domain} & Task 1 & Measurement 1 & \multirow{-2}{*}{loss} & \multirow{-2}{*}{\href{https://github.com/moukamisama/Recon}{\textcolor{citegreen}{Official}}}\\

        
    % \midrule % template
    %     \multirow{2}{*}{Model Name} & \multirow{2}{*}{Origin} & \multirow{2}{*}{Year} & MTL Strategy 1 & \multirow{2}{*}{Backbone} & \multirow{2}{*}{H/S} & \multirow{2}{*}{Domain} & Task 1 & Measurement 1 & \multirow{2}{*}{loss} & \multirow{2}{*}{\href{https://github.com}{\textcolor{citegreen}{XXXXX}}}\\
        
    %     & & & MTL Strategy 2 & & & & task 2  & measure 2 & & \\

    \bottomrule
    \end{tabular}
    % \caption{Caption}
    \label{tab:deep-sum}
    \begin{tablenotes}
    \footnotesize
    \item[1] This column provides the link to the implementation or execution. Click on "\textcolor{citegreen}{Official}" or "\textcolor{reforange}{Unofficial}" to access the website.
    \item[2] Part of PASCAL in Detail Workshop Challenge, CVPR 2017, July 26th, Honolulu, Hawaii, USA. \href{https://www.robots.ox.ac.uk/~vgg/decathlon/}{https://www.robots.ox.ac.uk/$\sim$vgg/decathlon}.
    \item[3] We use ``state" here to represent the domain of reinforcement learning, including the observations of states of environment, the positions of object, the actions made by agent, etc.
    \item[4] The average rank of MTL on all different tasks. MR = 1 if a method ranks first across all tasks.
    \end{tablenotes}
    \end{threeparttable}
    }
\end{table*}

% Multi-task Transformer
% https://github.com/prismformore/Multi-Task-Transformer




